Towards a Theory of Glue

We propose and study the notions of behaviour type and composition operator making a first step towards the definition of a formal framework for studying behaviour composition in a setting sufficiently general to provide insight into how the component-based systems should be modelled and compared. We illustrate the proposed notions on classical examples (Traces, Labelled Transition Systems and Coalgebras). Finally, the definition of memoryless glue operators, takes us one step closer to a formal understanding of the separation of concerns principle stipulating that computational aspects of a system should be localised within its atomic components, whereas coordination layer responsible for managing concurrency should be realised by memoryless glue operators.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{M. Carbone, I. Lanese, A. Silva, A. Sokolova (Eds.):\\
5th Interaction and Concurrency Experience (ICE'12).\\
EPTCS 104, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.104.6}{10.4204/EPTCS.104.6}}

